Spin-Weighted Spherical Harmonics for Polarized Light Transport

The objective of polarization rendering is to simulate the interaction of light with materials exhibiting polarization-dependent behavior. However, integrating polarization into rendering is challenging and increases computational costs significantly. The primary difficulty lies in efficiently modeling and computing the complex reflection phenomena associated with polarized light. Specifically, frequency-domain analysis, essential for efficient environment lighting and storage of complex light interactions, is lacking. To efficiently simulate and reproduce polarized light interactions using frequency-domain techniques, we address the challenge of maintaining continuity in polarized light transport represented by Stokes vectors within angular domains. The conventional spherical harmonics method cannot effectively handle continuity and rotation invariance for Stokes vectors. To overcome this, we develop a new method called polarized spherical harmonics (PSH) based on the spin-weighted spherical harmonics theory. Our method provides a rotation-invariant representation of Stokes vector fields. Furthermore, we introduce frequency domain formulations of polarized rendering equations and spherical convolution based on PSH. We first define spherical convolution on Stokes vector fields in the angular domain, and it also provides efficient computation of polarized light transport, nearly on an entry-wise product in the frequency domain. Our frequency domain formulation, including spherical convolution, led to the development of the first real-time polarization rendering technique under polarized environmental illumination, named precomputed polarized radiance transfer, using our polarized spherical harmonics. Results demonstrate that our method can effectively and accurately simulate and reproduce polarized light interactions in complex reflection phenomena.

==> app_s2l2.tex <==
\subsection{Stokes vector interpolation}
\label{sec:app-s2l2}
\dgkim{Isn't it better that section name should be ``Numerically stable representation'' or just ``S2L2 representation''? }
\NEWM{As described in Section~\ref{sec:stokes-on-sphere}, measuring Stokes vector suffers from non-deterministic choice of a local frame.
Also, due to the singularity problem of frame field, it shows numerically unstable behavior near by the singular point of frame field.
To overcome these problems, we found that PSH (in particular, spin-2 SH part) can provide numerically stable representation for Stokes vector.
}

\OLD{While polarized spherical harmonics provides benefit to construct a frequency domain framework on Stokes vector fields by encoding an entire polarized environment map or pBRDF into PSH coefficients, we also found another direction of application. Recall that conventionally measuring a Stokes vector suffers from nondeterministic choice of a local frame and numerical instability around frame field singularity. In this context, we found that spin-2 SH provides a numerically stable representation of not only Stokes vector fields, but also single Stokes vectors.
}

\NEWM{Suppose that we have a spin-2 Stokes vector $\dvs \in \STKsp{\homega}^2$.
By considering $\dvs$ as a Dirac delta Stokes vector field, we can project it to the frequency domain using PSH and taking its PSH coefficients up to order $l=2$.
As a result, we can represent $\dvs$ as a finite number of coefficient vector.
We named this representation as \emph{S2L2 representation}, defined as
}

\OLD{Suppose that we have a spin-2 Stokes vector $\dvs \in \STKsp{\homega}^2$. Considering a single Stokes vector $\dvs$ as a Dirac delta Stokes vector field and taking its PSH coefficients for order $l=2$, we define its novel representation, named \emph{S2L2 representation} as follows.
}

\begin{szTitledBox}{S2L2 representation of a Stokes vector}
	\vspace{-1mm}
	\begin{align} \label{eq:app-s2l2-def}
		\mathrm{S2L2}\left(\dvs\right) &=  \sqrt\frac{4\pi}{5}\begin{bmatrix}
			\lrangle{\dvY_{2-21}\left(\homega\right), \dvs}_\calS \\
			\lrangle{\dvY_{2-22}\left(\homega\right), \dvs}_\calS \\
			\vdots \\
			\lrangle{\dvY_{221}\left(\homega\right), \dvs}_\calS \\
			\lrangle{\dvY_{222}\left(\homega\right), \dvs}_\calS
		\end{bmatrix} \\ \nonumber
		&= \sqrt\frac{4\pi}{5}\begin{bmatrix}
		\R^2\left(\sY{2-2}\left(\theta,\phi\right)^* \C\left(\left[\dvs\right]^{\frF_{\theta\phi}\left(\theta,\phi\right)}\right)\right) \\
		\vdots \\
		\R^2\left(\sY{22}\left(\theta,\phi\right)^* \C\left(\left[\dvs\right]^{\frF_{\theta\phi}\left(\theta,\phi\right)}\right)\right)
		\end{bmatrix} \in \R^{10},
	\end{align}
	\vspace{-2mm}
\end{szTitledBox}
\NEWM{\noindent where the name S2L2 comes from \emph{spin-2} and PSH order $l=2$.
For the derivation of normalization constant  $\sqrt{4\pi / 5}$, refer Equation~\eqref{supp-eq:app-s2l2-norm} in supplemental material.
Note that we used 10-dimensional real-valued numeric vector in Equation~\eqref{eq:app-s2l2-def}, but it is also possible to represent it by 5-dimensional complex-valued numeric vector by combining the $s_1$ and $s_2$ components.

Conversely, the inverse of S2L2 representation, which reconstruct spin-2 Stokes vector $\dvs\in\STKsp{\homega}^2$ from given S2L2 representation $\bfr = \begin{bmatrix}r_1& \cdots& r_{10}\end{bmatrix}^T\in\R^{10}$ can be defined as
\begin{szTitledBox}{Stokes vector from S2L2 representation}
	\vspace{-1mm}
		\begin{align}\label{eq:app-s2l2-inv}
			\mathrm{S2L2Inv}\left(\bfr; \homega\right) &=  \sqrt\frac{4\pi}{5}\sum_{m=-2}^2 \sum_{p=1}^2 r_{2\left(m+2\right)+p}\, \dvY_{2mp}\left(\homega\right) \\ \nonumber
			&= \sqrt\frac{4\pi}{5}\left[\sum_{m=-2}^2 \tilde r_{m+3} \, \sY{2m}\left(\theta,\phi\right) \right]_{\frF_{\theta\phi}\left(\theta,\phi\right)} \in \STKsp{\homega}.
		\end{align}
	\vspace{-2mm}
\end{szTitledBox}
\noindent Then for any Stokes vector $\dvs\in\STKsp{\homega}$,
\begin{equation} \nonumber
	\mathrm{S2L2Inv}\left(\mathrm{S2L2}\left(\dvs\right); \homega\right)=\dvs
\end{equation}
\noindent holds. On the other hand, the equality $\mathrm{S2L2}\left(\mathrm{S2L2Inv}\left(\bfr;\homega\right)\right)=\bfr$ holds only if $\bfr$ is the S2L2 representation of some Stokes vector in $\STKsp{\homega}$, since $\R^{10}$ is a much larger set than $\calS$. If we have $\bfr\notin \mathrm{S2L2}\left(\calS\right)$, out of the range of the function $\mathrm{S2L2}$, $\mathrm{S2L2Inv}\left(\bfr; \homega\right)$ projects the input to a suitable Stokes vector.\dgkim{Unclear statement}


Since S2L2 representation is defined based on PSH, the S2L2 representation itself is continuous and independent to the choice of frame fields.
In other words, a small amount of perturbation on Stokes vector will change small amount of S2L2 value, and there is no singular point that causes the numerical instability.
Therefore, using the S2L2 representation can lead to stable numerical computation.
This property is important when we do some computational applications using polarized lights. 
As a best of our knowledge, this is the first continuous representation of Stokes vector in terms of numeric quantity.

\dgkim{Do we need this? It seems this distance part is mostly for numerical validations. Both numerical validation part and distance part is more suitable for supplemental, and here we just mention we validated it}
On the other hand, S2L2 representation allows us to define the distance between two Stokes vectors even if they are not defined along identical ray direction, based on its frame-independent property.
For two Stokes vectors $\dvs\in\STKsp{\homega_1}$ and $\dvt\in\STKsp{\homega_2}$, the distance between them is defined as
\begin{equation}\label{eq:app-s2l2-distance}
	d_{\mathrm{S2L2}}\left(\dvs, \dvt\right) = \norm{\mathrm{S2L2}\left(\dvs\right) - \mathrm{S2L2}\left(\dvt\right)}_2.
\end{equation}
Thanks to the rotation invariance of PSH, this distance is also rotation invariant, which can be written as
\begin{equation}
	d_{\mathrm{S2L2}}\left(\dvs, \dvt\right) = d_{\mathrm{S2L2}}\left(\vec R_\calS\dvs, \vec R_\calS\dvt\right),
\end{equation}
where $\vec R\in\SOgroupv$ is an arbitrary rotation.
It guarantees that further application methods based on S2L2 representation can produce consistent results even if we take different global frame, which assign spherical coordinates with a different north pole $\hat z_g$.
}

\OLD{
\noindent The name \emph{S2L2} indicates \emph{spin-2} and the order $l=2$. Here, we have an additional normalization constant $\sqrt{4\pi / 5}$ (Supp. Equation~\eqref{supp-eq:app-s2l2-norm}). Note that from the right hand side we can also define the value of $\mathrm{S2L2}\left(\dvs\right)$ as an element in $\C^5$ as an alternative choice. Encoding a full Stokes vector including $s_0$ intensity and $s_3$ circular polarization can be done by directly concatenating them to the resulting numeric vector of Equation~\eqref{eq:app-s2l2-def}.

The S2L2 representation satisfies nice properties which cannot be satisfied by representing Stokes components under a choice of a frame field. First, as best of our knowledge, it is the first continuous representation of Stokes vectors into $\R^n$ independent of choices of local frames. In other words, if we perturb a Stokes vector with small amount then the resulting S2L2 values changes with only a small amount. This property gives us numerical stability for computing polarized light transport.

In application perspective, the S2L2 representation allows us to define distance between two Stokes vector even if they are not defined along identical ray direction. For two Stokes vectors $\dvs\in\STKsp{\homega_1}$ and $\dvt\in\STKsp{\homega_2}$, we define the distance between them as
\begin{equation}\label{eq:app-s2l2-distance}
	d_{\mathrm{S2L2}}\left(\dvs, \dvt\right) = \norm{\mathrm{S2L2}\left(\dvs\right) - \mathrm{S2L2}\left(\dvt\right)}_2.
\end{equation}
The second noticeable property of S2L2 representation is that this distance is rotation invariant, i.e. $d_{\mathrm{S2L2}}\left(\dvs, \dvt\right) = d_{\mathrm{S2L2}}\left(\vec R_\calS\dvs, \vec R_\calS\dvt\right)$ for any rotation transform $\vec R\in\SOgroupv$. It guarantees that further application methods based on S2L2 representation can produces consistent results even if we take different global frame so that assign spherical coordinates with a different north pole $\hat z_g$.
}

\begin{figure}[tbp]
	\centering
	\includegraphics[width=\columnwidth]{figs/app_s2l2_perturb.pdf}%
	\vspace{-2mm}
	\caption[]{\label{fig:app_s2l2_perturb}
		We propose a novel representation for Stokes vectors, named \emph{S2L2 represenation}. We numerically validate our method compared with Stokes components representation under $\theta\phi$ frame field and a frame field introduced by \citet{durand2005frequency}, respectively. (a)., which provides numerical stability (a, b) under small perturbation of Stokes vectors and rotation invariant distance (c, d). Note that since we are testing with unit-norm Stokes vectors, the value 2.0 in x axes can be considered as the possible maximum value.}
	\vspace{-4mm}		
\end{figure}

\paragraph{Continuity validation}
While the continuity of S2L2 and rotation invariance of $d_\mathrm{S2L2}$ come from their definition, we also provide a numerical experiment to validate these properties and our implementation. First, we generated a set of spin-2 Stokes vectors, denoted by $S$. To make elements in $S$ uniformly distributed, we choose $N=1000$ ray directions $\homega_1...\homega_N\in\Sspv$ by spherical Fibonacci point set~\cite{svergun1994solution,hannay2004fibonacci}. For each $\homega_i$, we take four directions of Stokes component vectors as $\left[1, 0\right]^T$, $\left[0, 1\right]^T$, $\left[-1, 0\right]$, and $\left[0, -1\right]^T$ with $\theta\phi$ frame field so that $S$ consists of $4N$ spin-2 Stokes vectors. For each $\dvs\in S$, as described in Figure~\ref{fig:app_s2l2_perturb}(a), we perturbed it by rotating around each axis $\homega_1...\homega_N$ by $0.1\,\mathrm{rad}$, i.e., $\vec R_i = \vec R_{\homega_i}\left(0.1\, \mathrm{rad}\right)$. To measure how much change in numerical representation occurs from $0.1\, \mathrm{rad}$ perturbation, we collect $\max_{\vec R_i} d\left(\dvs, \vec R_{i\calS}\dvs\right)$ for each $\dvs \in S$ and plot its histogram in Figure~\ref{fig:app_s2l2_perturb}(b). To compare with conventional representation using frame fields, we uses the distance in Stokes component vectors as
\begin{equation}\nonumber
	d_{\frF}\left(\dvs,\dvt\right) = \norm{\left[\dvs\right]^{\frF} - \left[\dvt\right]^{\frF}}_2,
\end{equation}
for the first and second plots in Figure~\ref{fig:app_s2l2_perturb}(b). We are using $\theta\phi$ frame field and a frame field introduced by \citet{duff2017building}, which has been used in recent polarized graphics research~\cite{Mitsuba3, kim2023nespof}, for the first and second plots, respectively. Our S2L2 distance in Equation~\eqref{eq:app-s2l2-distance} is tested in the third plot. We observe that the maximum distances due to perturbation for each Stokes vector have non-uniform distance under frame field representation as seen in the first and second plots in Figure~\ref{fig:app_s2l2_perturb}(b). In addition, several Stokes vectors change their representation by amount `2', which indicates the opposite directions of Stokes component vectors since we are using unit-norm Stokes component vectors $\left[1,0\right]^T,...,\left[-1,0\right]^T$ as stated above. It is raised around frame field singularities. On the other hand, our representation yields a uniform values at $0.2$, which is ten times smaller than largest distances in the first and second plots, within just a negligible error $\pm10^{-14}$.

\paragraph{Rotation invariance validation}
We also tested how much rotation invariant each representation is. For each pair of Stokes vectors $\dvs, \dvt\in S$, as illustrated in Figure~\ref{fig:app_s2l2_perturb}(c), we are measuring how much the distance between them changes under rotations, as $\max_{\vec R}\abs{d\left(\vec R_{\calS}\dvs, \vec R_{\calS}\dvt\right) - d\left(\dvs, \dvt\right)}$. Here, wa are taking maximum over each rotation in $\vec R = \vec R_{\homega_i}\left(\theta_j\right)$ where $\theta_j$ takes values from 10 uniformly spaced values in $\left[0, 2\pi\right)$. Collecting the maximum distance change over each rotation transform for each Stokes vector $\dvs \in S$, its histogram is shown in Figure~\ref{fig:app_s2l2_perturb}(d). We clearly observe that the first and second plots which using distances induced by frame fields representation have large change of distance under rotation, but in the third plot, our S2L2 representation gives actually rotation invariant representation of Stokes vectors, within just a negligible error $7.69\times 10^{-14}$.


\OLD{\paragraph{Stokes vectors from S2L2 representation}
As a converse of S2L2 representation introduced in Equation~\eqref{eq:app-s2l2-def}, if we have a S2L2 representation $\bfr = \begin{bmatrix}r_1& \cdots& r_{10}\end{bmatrix}^T\in\R^{10}$ (or $\tilde \bfr = \begin{bmatrix}\tilde r_1& \cdots& \tilde r_5\end{bmatrix}^T\in \C^5$, equivalently) then we can reconstruct the unknown spin-2 Stokes vector $\dvs\in\STKsp{\homega}^2$ as follows.
\begin{szTitledBox}{Stokes vector from S2L2 representation}
	\vspace{-1mm}
		\begin{align}\label{eq:app-s2l2-inv}
			\mathrm{S2L2Inv}\left(\bfr; \homega\right) &=  \sqrt\frac{4\pi}{5}\sum_{m=-2}^2 \sum_{p=1}^2 r_{2\left(m+2\right)+p}\, \dvY_{2mp}\left(\homega\right) \\ \nonumber
			&= \sqrt\frac{4\pi}{5}\left[\sum_{m=-2}^2 \tilde r_{m+3} \, \sY{2m}\left(\theta,\phi\right) \right]_{\frF_{\theta\phi}\left(\theta,\phi\right)} \in \STKsp{\homega}.
		\end{align}
	\vspace{-2mm}
\end{szTitledBox}
\noindent Then for any Stokes vector $\dvs\in\STKsp{\homega}$,
\begin{equation} \nonumber
	\mathrm{S2L2Inv}\left(\mathrm{S2L2}\left(\dvs\right); \homega\right)=\dvs,
\end{equation}
\noindent holds. On the other hand, the equality $\mathrm{S2L2}\left(\mathrm{S2L2Inv}\left(\bfr;\homega\right)\right)=\bfr$ holds only if $\bfr$ is the S2L2 representation of some Stokes vector in $\STKsp{\homega}$, since $\R^{10}$ is a much larger set than $\calS$. If we have $\bfr\notin \mathrm{S2L2}\left(\calS\right)$, out of the range of the function $\mathrm{S2L2}$, $\mathrm{S2L2Inv}\left(\bfr; \homega\right)$ projects the input to a suitable Stokes vector. One of reason that we denote $\mathrm{S2L2Inv}$ rather than $\mathrm{S2L2}^{-1}$ is that there can be other choices to evaluate such projection in future work, and we are providing one baseline choice as $\mathrm{S2L2Inv}$, defined in Equation~\eqref{eq:app-s2l2-inv}.
}

\begin{figure*}[tpb]
	\centering
	\includegraphics[width=\textwidth]{figs/app_s2l2_result.pdf}%
	\vspace{-3mm}
	\caption[]{\label{fig:app_s2l2_result}
		Our frame-free S2L2 representation for Stokes vectors provides a numerically stable and artifact-free resampling (warping) methods for polarized environment maps.
		In this experiment, starting from a cubemap polarized environment map obtained by Mitsuba 3 renderer with six poses for perspective cameras, (i) we first resample it into a equirectanguler image, under Stokes component vector representation under $\theta\phi$ frame field and our S2L2 representation for (b) and (c), respectively. 
		(b) yields an artifact in $s_1$ component (green boxed close up), violation of two rotation property, described in Figure~\ref{fig:bkgnd_continuity_stokes_field}(b), at the top row (purple boxed plot), and incorrect result for intensity through a longitudinal polarizer (blue boxed close up), our results in (c) provides an artifactless correct equirectangular images. 
		In the next step of the experiment, (ii) we once more resample the equirectangular images into a perspective view. Here we can clearly observe that (b) yields severe artifacts while our result (c) produces artifactless images.}
	\vspace{-2mm}		
\end{figure*}

\NEWM{Based on the S2L2 and its inverse representation defined, now we can define an interpolation between two Stokes vectors using S2L2 representation.
Suppose that there are two Stokes vector $\dvs\in\STKsp{\homega_1}$ and $\dvt\in\STKsp{\homega_2}$.
Thanks to the frame independent nature of S2L2 representation, the interpolation can be defined using S2L2 representation even two Stokes vectors belong different Stokes space, i.e., $\homega_1\ne \homega_2$.
This interpolation can be written as
\begin{equation}\label{eq:app-s2l2-interp}
	\mathrm{S2L2Inv}\left(\left(1-\alpha\right)\mathrm{S2L2}\left(\dvs\right) + \alpha\mathrm{S2L2}\left(\dvt\right); \homega\left(\alpha\right)\right),
\end{equation}
where $\homega\left(\alpha\right)$ indicates an interpolation of $\homega_1$ and $\homega_2$, such as linear interpolation or axis-angle based rotation interpolation.
}

\OLD{
The such projection provides another fundamental application, Stokes vector interpolation. For two Stokes vector $\dvs\in\STKsp{\homega_1}$ and $\dvt\in\STKsp{\homega_2}$, we can define an interpolation of them even if they belong to different Stokes spaces, i.e. $\homega_1\ne \homega_2.$ as follows.

\begin{equation}\label{eq:app-s2l2-interp}
	\mathrm{S2L2Inv}\left(\left(1-\alpha\right)\mathrm{S2L2}\left(\dvs\right) + \alpha\mathrm{S2L2}\left(\dvt\right); \homega\left(\alpha\right)\right),
\end{equation}
where $\homega\left(\alpha\right)$ indicates an interpolation of $\homega_1$ and $\homega_2$ which is up to implementation details, such as $\homega\left(\alpha\right)=\mathrm{normalzie}\left(\left(1-\alpha\right)\homega_1 - \alpha\homega_2\right)$. 
Note that as $d_{\mathrm{S2L2}}$ in Equation~\eqref{eq:app-s2l2-distance} does, our Stokes vector interpolation in Equation~\eqref{eq:app-s2l2-interp} satisfies continuous change of Stokes vectors and rotation invariance.
}

\NEWM{One important application of Stokes vector interpolation is the Stokes image resampling.
Figure~\ref{fig:app_s2l2_result} shows the experiment setup and result of Stokes image resampling.
We first render 6 perspective images with polarization components.
All 6 camera have 90\degree\ field-of-view, and the pose of each camera is set to capture whole surrounding environment, which leads to capture a cubemap described in Figure~\ref{fig:app_s2l2_result}(a).
Then we conduct two resampling experiments, resample the equirectangular image from the cubemap and resample the single perspective image again from the resampled equirectangular image.
As a result, we obtain image size of six $64\times64$ for the cubemap and $1024\times 2048$ for the equirectangular image, and $64\times64$ for the resampled perspective image.
We compare our method in Equation~\eqref{eq:app-s2l2-interp} with the conventional approach, which represent Stokes vectors as numeric Stokes components under a certain frame field.
Figure~\ref{fig:app_s2l2_result}(b) and (c) indicates the results of the conventional approach using $\theta\phi$ frame field and using our proposed S2L2 interpolation, respectively.
}

\OLD{
While our Stokes vector interpolation is simple but general so that it can be used to various potential applications, we introduce image resampling results here. Note that there are many way to visualize environment maps. We are testing resampling between perspective views, including cube maps, and equirectangular images, as described in Figure~\ref{fig:app_s2l2_result}(a). Starting from cube map images obtained by rendering a 3D scene with six camera poses, we resampling it into Figure~\ref{fig:app_s2l2_result}(i) equirectangular images, and then Figure~\ref{fig:app_s2l2_result}(ii) ressample them into a single perspective view again. We compare our method in Equation~\eqref{eq:app-s2l2-interp} with a conventional approach which represent Stokes vectors as numeric Stokes components under a certain frame field. Figure~\ref{fig:app_s2l2_result}(b) and (c) indicates the results of the conventional approach using $\theta\phi$ frame field in Equation~\eqref{eq:movingf_tp} and ours, respectively.
}

\dgkim{Why not using same setup (256)? Also, we can mention just image resolutions in one sentence. Or just mention it in the caption of the image.}
\OLD{
Note that to make difference of both methods more visible, we are testing upsampling $6\times 64\times 64$ cube map images to $1024\times 2048$ equirectangular images in (b)(i) and (c)(i), while (a)(i) shows the image resampled from a high resolution $6\times 1024\times 1024$ cube map for ground truth. Similarly, (b)(ii) and (c)(ii) indicate resampled $256\times256$ images from (b)(i) and (c)(i), respectively, while images in (a)(ii) are originally rendered ones without resampling.
}

\dgkim{This paragraph needs substantial rewriting. First, there is too much label and it is also not organized. This part is very important so the clear explanation is necessary. Second, It is very hard to recognize what is important part. One paragraph should include ONE statement. Although I can recognize what is what and how to understand the figure and this paragraph, but maybe reviewer will complain about this.}
From (b)(i) and (c)(i) we can see that conventional approach yields an artifact in the $s_1$ component image but ours produces cleaner image. However, it is hard to compare these results with ground truth since interpolation between Stokes vectors with different ray directions has not been have such a ground truth definition. Instead, we validate results in (b)(i) and (c)(i) in two ways. First, we can check the top row of equirectangular images, which indicates an nonzero polarized illumination at the center point in the perspective image in (ii). We can plot $\left(s_1,s_2\right)$ component values for each $\phi$ and check whether it follows the two rotation property described at the bottom plot with cyan colored curved in Figure~\ref{fig:bkgnd_continuity_stokes_field}(b)\footnote{It corresponds to $\theta=\pi$ rather than $\theta=0$ due to the convention of visualizing environment maps. See Supp. Figure~\ref{supp-fig:envmap-convention}(b).}. In the plot with a purple boundary in Figure~\ref{fig:app_s2l2_result}(b)(i) we can see the conventional approach yields a wrong zero value but ours in (c)(i) produces nonzero value with the two rotation property. Second, if we convert Stokes vector images into scalar images through a polarizer then we can compare it with a ground truth resampled result. If we take $\frac{s_0+s_1}{2}$ images for (b)(i) and (c)(i) then it should be identical to a scalar environment map obtained by rendering the scene with append a sphere-shaped polarized with longitudinal direction at the projection center of the camera, which is shown in the top rightmost image in (a)(i). Then we can see in (b)(i) the artifact in the intensity through longitudinal polarizer using conventional approach is wrong compared with GT in (a)(i), but ours in (c)(i) is more closer to GT.

After resampling equirectangular images into a perspective view, we can see the artifact in (b)(ii) more clearly. However, our result in (c)(ii) yields cleaner image through numerically stable computation. Note that while we are testing conventional approach with a $\theta\phi$ frame field, using other frame field also yields such artifact at different positions of the singularity.




==> application1.tex <==
\section{Application 1: Real-time Polarized Rendering}
\label{sec:prt}
\subsection{Previous work on SH rendering for scalar radiance}
\cite{ramamoorthi2001efficient}, \cite{sloan2002precomputed}, ..

\subsection{Implementation details}
\SHIN{TBA}

\subsection{Results}
Figure~\ref{fig:app_prt_result}








==> application2.tex <==
8%



\section{Application 2: Polarized Radiance Fields with Spin-2 SH}

To show variety of application of spin-2 spherical harmonics which is not only limited to forward rendering methods, here we present the first polarized radiance field method as another application. To inherit frequency domain framework for novel view synthesis, we propose a polarized version of Plenoxels~\cite{yu_and_fridovichkeil2021plenoxels}.
\SHIN{Overview diagram figure}
\subsection{Plenoxels}
From a set of posed images, Plenoxels~\cite{yu_and_fridovichkeil2021plenoxels} optimizes a sparse voxel grid with density $\sigma$ and spherical harmonic coefficients at each voxel. The spherical harmonic coefficients are used to obtain a view dependent radiance $\mathbf{c}$.
Via volume rendering~\cite{kajiya1984ray,drebin1988volume}, we can render a ray from a Plenoxel model:
\begin{align}
\label{eq:volume_rendering}
\hat{\mathbf{C}}(\mathbf{r}) &= \sum_{i=1}^{N} T_i(1-\text{exp}(-\sigma_i\delta_i))\mathbf{c}_i,\\
T_i &= \text{exp}\left(-\sum_{i-1}^{j}\sigma_j\delta_j\right),
\end{align}
where $\delta_i$ is the distance between two consecutive sample points and $N$ is the number of samples along the ray, and $T_i$ indicates the accumulated transmittance along the ray. 
We optimize the density field and the spherical harmonic coefficients using the input color $\mathbf{C}$ as supervision:
\begin{equation}
\mathcal{L} = \left \| \hat{\mathbf{C}}(\mathbf{r}) - \mathbf{C}(\mathbf{r}) \right \|_{2}^{2}.
\label{eq:photometric_loss}
\end{equation}

\subsection{Polarized Radiance as spin-2 SH}
To allow Plenoxels to handle Stokes vectors, we start by treating $s_0$ as it is in the original implementation: given a voxel and a view direction, we estimate the color using the nine coefficients corresponding to $l\in\llbracket0, 2\rrbracket$ for the conventional spherical harmonics. 
For the Stokes coefficients $s_1$ and $s_2$, we use pin-2 SH with $l=2$, hence five spherical harmonic coefficients for each Stokes coefficient and color channel.
Note that we only use $s_0$ to optimize the density.
For our experiments, we optimize a 256$^\text{3}$ voxel grid for 512000 iterations. 

\subsection{Results}
We build a synthetic polarized dataset based on three of Nerf's Blender scenes~\cite{mildenhall2020nerf}. For polarization-aware rendering, we convert the scenes to Mitsuba3~\cite{Mitsuba3}, change BSDF types to polarization-aware ones, add polarizers against the light sources and render with Mitsuba3's polarized variant.
We compare our approach against Naïve SH, which indicates naïvly appying conventional SH to Stokes components with respect to the $\theta,\phi$-moving frame, similar to Figure~\ref{fig:bkgnd_continuity_stokes_field} (b).
Table~\ref{tb:plenoxels} shows mean square error for the linear components of the Stokes maps ($s_1$ and $s_2$) on non-transparent pixels and Figure~\ref{fig:plenoxels} shows the linear polarization components of the Stokes maps at novel views.

\begin{figure*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{1pt}
	\renewcommand{\arraystretch}{0.6}
	\begin{tabular}{cccccccccc}
		\centeredtab{\rotatebox[origin=c]{90}{P-Materials}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/gt_0000_S0.jpg}} &
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/gt_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/naive/pred_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/s2sh/pred_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/gt_0000_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/naive/pred_0000_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/s2sh/pred_0000_S2_cm.jpg}} &
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/naive/err_0000.jpg}} & 
		\centeredtab{\includegraphics[trim={60px 280px 390px 200px},clip,width=0.105\textwidth]{figs/plenoxels/materials/s2sh/err_0000.jpg}}
		\\
		\centeredtab{\rotatebox[origin=c]{90}{P-Lego}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/gt_0100_S0.jpg}} &
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/gt_0100_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/naive/pred_0100_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/s2sh/pred_0100_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/gt_0100_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/naive/pred_0100_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/s2sh/pred_0100_S2_cm.jpg}} &
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/naive/err_0100.jpg}} & 
		\centeredtab{\includegraphics[trim={250px 210px 250px 350px},clip,width=0.105\textwidth]{figs/plenoxels/lego/s2sh/err_0100.jpg}}
		\\
		\centeredtab{\rotatebox[origin=c]{90}{P-Hotdog}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/gt_0000_S0.jpg}} &
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/gt_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/naive/pred_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/s2sh/pred_0000_S1_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/gt_0000_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/naive/pred_0000_S2_cm.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/s2sh/pred_0000_S2_cm.jpg}} &
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/naive/err_0000.jpg}} & 
		\centeredtab{\includegraphics[trim={240px 300px 250px 190px},clip,width=0.105\textwidth]{figs/plenoxels/hotdog/s2sh/err_0000.jpg}}
		\\
        & RGB (GT) & $s_1$ (GT) & $s_1$ (Naïve) & $s_1$ (Spin-2 SH) & $s_2$ (GT) & $s_2$ (Naïve) & $s_2$ (Spin-2 SH) & Error (Naïve) & Error (Spin-2 SH) \\
	\end{tabular}
	\caption{\textbf{Polarized Radiance Fields Results Close-ups.}
		The P-Lego scene clearly shows naïve SH's discontinuity when the view direction is aligned with the $z$ axis. P-Material shows that this discontinuity makes optimization unstable, even for angles far from the $z$ axis. Non-cropped results are available in the supplemental document.
	}
	\label{fig:plenoxels}
\end{figure*}

\begin{table}[tbp]\small
	\caption{\label{tb:plenoxels} 
	\textbf{Polarized Radiance Fields Results.} We report MSE on our synthetic dataset. Spin-2 SH shows consistently lower error than naïve spherical harmonics.}
	\vspace{-3mm}
	\begin{tabular}{l r r r}
		\toprule
		Scene & P-Materials & P-Lego & P-Hotdog \\ 
		\midrule
		Naïve 		& $			3.59\cdot10^{-2}$ & $			1.97\cdot10^{-3}$ & $			1.16\cdot10^{-2}$ \\
		Spin-2 SH 	& $\mathbf{	2.03\cdot10^{-2}}$ & $\mathbf{	1.45\cdot10^{-3}}$ & $\mathbf{	9.55\cdot10^{-3}}$ \\
		\bottomrule
	\end{tabular}
\end{table}


==> applications.tex <==
\section{Applications}
\label{sec:application}

TBA application


==> equation_table_symmetry.tex <==







==> from-main.tex <==













==> notations.tex <==
\begin{table}[tbp]\small
	\caption{\label{tb:sets_arith} 
		Symbols for sets and arithmetics.}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.25\linewidth} m{0.65\linewidth}} %
		\thickhline
		Symbol   & Description \\ \thickhline
		
		$\R, \C$ & the set of all real / complex numbers\\
		$z^*=x-yi$ & complex conjugation of $z=x+yi\in\C$ \\
		$\Re z = x$ & the real part of $z=x+yi\in\C$\\
		$\Im z = y$ & the imaginary part of $z=x+yi\in\C$\\
		\hline
		$\R^2\left(z\right)=\left[x, y\right]^T$ & conversion from a complex number $z=x+yi$ to a 2D real numeric vector \\
		$\C\left(\left[x,y\right]^T\right)=x+yi$ & conversion from a 2D real numeric vector to a complex number \\
		$\R^{2\times 2}\left(z\right)$ & conversion from a complex number $z$ to a $2\times 2$ real matrix, defined in Eq.~\eqref{eq:theory_comp2mat}. \\
		$\Ciso\left(\bfM\right), \Cconj\left(\bfM\right)$ & conversion from a $2\times 2$ real matrix $\bfM$ to two complex numbers resp., defined in Eq.~\eqref{eq:theory_mat2comp}. \\
		$\bfJ=\begin{bmatrix} 1&0 \\ 0&-1 \end{bmatrix}$ & a $2\times 2$ numeric matrix used to convert between $2\times 2$ matrices and pairs of complex numbers in Eq.~\eqref{eq:theory_mat2comp}. \\
		\hline
		
		\thickhline
		
		
		
	\end{tabular}
	
	
	\vspace{-3mm} 
\end{table}




\begin{table}[tbp]\small
	\caption{\label{tb:elem_set_desc} 
		Symbol definitions of sets of each type quantities, notation convention for their elements, and descriptions. Empty cells indicate \emph{they depend on context}.}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.13\linewidth} m{0.21\linewidth} m{0.51\linewidth}} %
		\thickhline
		Set & Element & Description \\ \thickhline
		
		$\R^3$&$\bfx,\bfy,\cdots$ & the space of 3D numeric vectors \\
		$\Rspv$ & $\vec x, \vec y,\cdots$&the space of 3D (geometric) vectors \\
		$\Sspv$ & $\homega,\cdots$&unit sphere, the set of all \textit{directions}, $=\!\left\{\vec x\!\in\!\Rspv\mid \norm{\vec x}\!=\!1\right\}$\\
		\hline
		
		$\calF\left(X, Y\right)$ && the function space from $X$ into $Y$, for given sets $X$ and $Y$ \\
		$\SOgroup $ & $\bfR,\cdots$ &the set of 3D rotation (numeric) matrices, $\subset \calL\left(\R^3,\R^3\right)$ \\
		$\SOgroupv $ & $\vec R,\cdots$ &the set of 3D rotation (geometric) transforms, $\subset \calL\left(\Rspv,\Rspv\right)$ \\
		$\FRsp $ &$\frF,\cdots$& the set of orthonormal frames in 3D, $\subset \calL\left(\R^3, \Rspv\right)$\\
		\thickhline
		
		
		
	\end{tabular}
	
	
	\vspace{-3mm} 
\end{table}


==> notations_all.tex <==
\begin{table}[tbp]\small
	\caption{\label{tb:sets_arith} 
		Symbols for sets and arithmetics.}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.25\linewidth} m{0.65\linewidth}} %
		\thickhline
		Symbol   & Description \\ \thickhline
		$\R, \C$
		& the set of all real / complex numbers\\
		
		$z^*=x-yi$
		& complex conjugation of $z=x+yi\in\C$ \\
		
		$\Re z = x$
		& the real part of $z=x+yi\in\C$\\
		
		$\Im z = y$
		& the imaginary part of $z=x+yi\in\C$\\
		
		\hline
		
		$\R^2\left(z\right)=\left[x, y\right]^T$
		& conversion from a complex number $z=x+yi$ to a 2D real numeric vector \\
		
		$\C\left(\left[x,y\right]^T\right)=x+yi$
		& conversion from a 2D real numeric vector to a complex number \\
		
		$\R^{2\times 2}\left(z\right)$
		& conversion from a complex number $z$ to a $2\times 2$ real matrix, defined in Eq.~\eqref{eq:theory_comp2mat}. \\
		
		$\Ciso\left(\bfM\right), \Cconj\left(\bfM\right)$
		& conversion from a $2\times 2$ real matrix $\bfM$ to two complex numbers resp., defined in Eq.~\eqref{eq:theory_mat2comp}. \\
		
		$\bfJ=\begin{bmatrix} 1&0 \\ 0&-1 \end{bmatrix}$ & a $2\times 2$ numeric matrix used to convert between $2\times 2$ matrices and pairs of complex numbers in Eq.~\eqref{eq:theory_mat2comp}. \\
		
		\hline
		
		
		\thickhline
	\end{tabular}
\end{table}




\begin{table}[tbp]\small
	\caption{\label{tb:elem_set_desc} 
		Symbol definitions of sets of each type quantities, notation convention for their elements, and descriptions. Empty cells indicate \emph{they depend on context}.}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.13\linewidth} m{0.21\linewidth} m{0.51\linewidth}} %
		\thickhline
		Set & Element & Description \\ \thickhline
		
		
		$\R^3$
		&$\bfx,\bfy,\cdots$
		& the space of 3D numeric vectors \\
		
		$\Rspv$
		&$\vec x, \vec y,\cdots$
		&the space of 3D (geometric) vectors \\
		
		$\Sspv$
		&$\homega,\cdots$
		&unit sphere, the set of all \textit{directions}, $=\!\left\{\vec x\!\in\!\Rspv\mid \norm{\vec x}\!=\!1\right\}$\\
		
		\hline
		
		$\calF\left(X, Y\right)$
		&
		&the function space from $X$ into $Y$, for given sets $X$ and $Y$ \\
		
		$\calL\left(X, Y\right)$
		&
		&the set of linear maps from $X$ into $Y$, for given linear spaces $X$ and $Y$ \\
		
		$\SOgroup $ 
		& $\bfR,\cdots$ 
		&the set of 3D rotation (numeric) matrices, $\subset \calL\left(\R^3,\R^3\right)$ \\
		
		$\SOgroupv $ 
		& $\vec R,\cdots$ 
		&the set of 3D rotation (geometric) transforms, $\subset \calL\left(\Rspv,\Rspv\right)$ \\
		
		$\FRsp $ 
		&$\frF,\cdots$
		& the set of orthonormal frames in 3D, $\subset \calL\left(\R^3, \Rspv\right)$\\
		
	
		
		\thickhline
	\end{tabular}
\end{table}




\begin{table}[tbp]\small
	\caption{\label{tb:polar_symbols} 
		Symbols and conventions about Mueller calculus
	}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.13\linewidth} m{0.77\linewidth}} %
		\thickhline
		Symbol   & Description \\ \thickhline
		
		$\STKsp{\homega}$
		& \textit{Stokes space} along $\homega\in\bbS^2$, i.e., the set of all Stokes vectors of a ray along $\homega$\\
		

		$\MUEsp{\homega_i}{\homega_o}$
		& \textit{Mueller space} from $\STKsp{\homega_i}$ to $\STKsp{\homega_o}$ \\
		
		\hline
		
		$\bfx,\bfy,\cdots$
		& (numeric) Stokes component vectors, $\in\R^4$ \\
		
		$\dvx, \dvy,\cdots$
		& (geometric) Stokes vectors, $\in\STKsp{\homega}$ \\
		
		$\bfA,\bfB,\cdots$
		& (numeric) Mueller matrices, $\in\R^{4\times 4}$ \\
		
		$\dvA, \dvB,\cdots$
		& (geometric) Mueller transforms, $\in\MUEsp{\homega_i}{\homega_o}$ \\
		
		\hline
		

		$\left[\bfs\right]_{\frF}$
		&  Stokes vector $\in\!\STKsp{\extColz{\frF}}$ which has a Stokes component vector $\bfs$ w.r.t. a frame $\frF$ \\
		
		
		$\left[\dvs\right]^{\frF}$
		&  Stokes component vector $\in\R^4$ of a Stokes vector $\dvs$ w.r.t. a frame $\frF$ \\
		
		
		$\left[\bfM\right]_{\frF_1\to\frF_2}$
		&  Mueller transform $\in\!\MUEsp{\extColz{\frF_1}}{\extColz{\frF_2}}$ which has a Mueller matrix $\bfM$ w.r.t. frames $\frF_1,\frF_2$ \\
		
		
		$\left[\dvM\right]^{\frF_1\to\frF_2}$
		& numeric Mueller matrix $\in\R^{4\times 4}$ of a Mueller transform $\dvM $ w.r.t. frames $\frF_1,\frF_2$ \\
		
		\thickhline
	\end{tabular}
\end{table}






\begin{table}[tbp]\small
	\caption{\label{tb:rot_inner} 
		Several types of rotations and inner products
	}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.15\linewidth} m{0.65\linewidth} m{0.10\linewidth}} %
		\thickhline
		Symbol   & Operand & Eq.\# \\
		
		\thickhline
		
		$\vec R \vec x$,\quad $\vec R \frF$
		& vector $\vec x\in \Rspv$, and frame $\frF\in\FRsp$
		& \\
		
		$\vec R_\calS\dvx$
		& Stokes vector $\dvx \in \calS$
		& Eq.~\eqref{eq:stokes_rotation} \\
		
		
		$\vec R_\calM \left[\dvM\right]$
		& Mueller transforms $\dvM \in \calM$
		& Eq.~\eqref{eq:theory_rot_mueller}\\
		
		
		$\vec R_\calF \left[f\right]\left(\homega\right)$
		& scalar field $f:\Sspv\to \C$
		& Eq.~\eqref{eq:bkgnd_rot_sph_func} \\
		
		
		$\vec R_\calF \left[\dvf\right]\left(\homega\right)$
		& Stokes vector field $\dvf:\Sspv\to\STKsp{\homega}$
		& Eq.~\eqref{eq:theory_rot_STKfield} \\
		
		\thickhline
		
		
		$\lrangle{\dvs_1, \dvs_2}_\calS$
		& Stokes vectors $\dvs_1,\dvs_2\in\STKsp{\homega}$ (identical direction)
		& Eq.~\eqref{eq:bkgnd-stokes-inner} \\
		
		
		$\lrangle{f, g}_{\calF}$
		& scalar fields $f,g:\Sspv\to \C$
		& Eq.~\eqref{eq:bkgnd_sh_coeff} \\
		
		
		$\lrangle{\dvf, \dvg}_{\calF} $
		& Stokes vector fields $\dvf,\dvg:\Sspv\to\STKsp{\homega}$
		& Eq.~\eqref{eq:inner_stokes_field}\\
		
		\thickhline
	\end{tabular}
\end{table}


==> notations_polar.tex <==
\begin{table}[tbp]\small
	\caption{\label{tb:polar_symbols} 
		Symbols and conventions about Mueller calculus
	}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.13\linewidth} m{0.77\linewidth}} %
	\thickhline
	Symbol   & Description \\ \thickhline
	
	$\STKsp{\homega}$ & \textit{Stokes space} along $\homega\in\bbS^2$, i.e., the set of all Stokes vectors of a ray along $\homega$\\
	$\MUEsp{\homega_i}{\homega_o}$ & \textit{Mueller space} from $\STKsp{\homega_i}$ to $\STKsp{\homega_o}$ \\
	
	\hline
	
	$\bfx,\bfy,\cdots$ & (numeric) Stokes component vectors, $\in\R^4$ \\
	$\dvx, \dvy,\cdots$ & (geometric) Stokes vectors, $\in\STKsp{\homega}$ \\
	$\bfA,\bfB,\cdots$ & (numeric) Mueller matrices, $\in\R^{4\times 4}$ \\
	$\dvA, \dvB,\cdots$ & (geometric) Mueller transforms, $\in\MUEsp{\homega_i}{\homega_o}$ \\
	
	\hline
	
	$\left[\bfs\right]_{\frF}$ &  Stokes vector $\in\!\STKsp{\extColz{\frF}}$ which has a Stokes component vector $\bfs$ w.r.t. a frame $\frF$ \\
	$\left[\dvs\right]^{\frF}$ &  Stokes component vector $\in\R^4$ of a Stokes vector $\dvs$ w.r.t. a frame $\frF$ \\
	$\left[\bfM\right]_{\frF_1\to\frF_2}$ &  Mueller transform $\in\!\MUEsp{\extColz{\frF_1}}{\extColz{\frF_2}}$ which has a Mueller matrix $\bfM$ w.r.t. frames $\frF_1,\frF_2$ \\
	$\left[\dvM\right]^{\frF_1\to\frF_2}$ & numeric Mueller matrix $\in\R^{4\times 4}$ of a Mueller transform $\dvM $ w.r.t. frames $\frF_1,\frF_2$ \\
	
	\thickhline
\end{tabular}

\end{table}





\begin{table}[tbp]\small
	\caption{\label{tb:rot_inner} 
		Several types of rotations and inner products
	}
	\vspace{-3mm}
	\rowcolors{2}{lightgray!0}{lightgray!60}
	\begin{tabular}{m{0.15\linewidth} m{0.65\linewidth} m{0.10\linewidth}} %
		\thickhline
		Symbol   & Operand & Eq.\# \\ \thickhline
		
		$\vec R \vec x$,\ \ \ \  $\vec R \frF$ & vector $\vec x\in \Rspv$, and frame $\frF\in\FRsp$ & \\
		$\vec R_\calS\dvx$ & Stokes vector $\dvx \in \calS$ & Eq.~\eqref{eq:stokes_rotation} \\
		$\vec R_\calM \left[\dvM\right]$ & Mueller transforms $\dvM \in \calM$ & Eq.~\eqref{eq:theory_rot_mueller}\\
		$\vec R_\calF \left[f\right]\left(\homega\right)$ & scalar field $f:\Sspv\to \C$ & Eq.~\eqref{eq:bkgnd_rot_sph_func} \\
		$\vec R_\calF \left[\dvf\right]\left(\homega\right)$ & Stokes vector field $\dvf:\Sspv\to\STKsp{\homega}$ & Eq.~\eqref{eq:theory_rot_STKfield} \\
		\thickhline
		
		$\lrangle{\dvs_1, \dvs_2}_\calS$ & Stokes vectors $\dvs_1,\dvs_2\in\STKsp{\homega}$ (identical direction) & Eq.~\eqref{eq:bkgnd-stokes-inner} \\
		$\lrangle{f, g}_{\calF}$ & scalar fields $f,g:\Sspv\to \C$ & Eq.~\eqref{eq:bkgnd_sh_coeff} \\
		$\lrangle{\dvf, \dvg}_{\calF} $ & Stokes vector fields $\dvf,\dvg:\Sspv\to\STKsp{\homega}$ & Eq.~\eqref{eq:inner_stokes_field}\\
		\thickhline

		
		
	\end{tabular}
	
\end{table}


==> ourmethod.tex <==

\section{Method}
\label{sec:ourmethod}
TBA method


==> result.tex <==

\section{Results}
\label{sec:results-applications}
Based on the theoretical building blocks of polarized spherical harmonics introduced in Section~\ref{sec:our_theory}, we propose two applications results.
First, as an application of PSH basis functions introduced in Section~\ref{sec:spin_sph_harm} and~\ref{sec:theory_rotinv}, we propose a novel representation of Stokes vectors which is independent of choice of local frames in Section~\ref{sec:app-s2l2}, which can be used in Stokes vector interpolation and polarized environment map resampling (warping).
Second, based on the frequency domain formulations from Section~\ref{sec:spin_sph_harm} to~\ref{sec:theory_conv}, we propose a precomputed polarized radiance transfer in Section~\ref{sec:pprt}, which achieves the first real-time polarized rendering taking polarized environment lighting into account.



